GSFF-SLAM: 3D Semantic Gaussian Splatting SLAM via Feature Field

Semantic-aware 3D scene reconstruction is essential for autonomous robots to perform complex interactions. Semantic SLAM, an online approach, integrates pose tracking, geometric reconstruction, and semantic mapping into a unified framework, shows significant potential. However, existing systems, which rely on 2D ground truth priors for supervision, are often limited by the sparsity and noise of these signals in real-world environments. To address this challenge, we propose GSFF-SLAM, a novel dense semantic SLAM system based on 3D Gaussian Splatting that leverages feature fields to achieve joint rendering of appearance, geometry, and N-dimensional semantic features. By independently optimizing feature gradients, our method supports semantic reconstruction using various forms of 2D priors, particularly sparse and noisy signals. Experimental results demonstrate that our approach outperforms previous methods in both tracking accuracy and photorealistic rendering quality. When utilizing 2D ground truth priors, GSFF-SLAM achieves state-of-the-art semantic segmentation performance with 95.03\% mIoU, while achieving up to 2.9$\times$ speedup with only marginal performance degradation.

==> tab/exp_replica_slam.tex <==
\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{2pt}
    \renewcommand{\arraystretch}{1.05}
    \newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l*{5}{C{2cm}}}
        \toprule
        Method & ATE RMSE$\downarrow$ & Depth L1$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$\\
        \midrule
        \multicolumn{6}{l}{\cellcolor[HTML]{EEEEEE}{\textit{Neural Implicit Fields}}} \\ 
        % 
        \multirow{1}{*}{NICE-SLAM~\cite{zhu2022nice}} 
        & 2.16& 3.09 & 25.24 & 0.813 & 0.221      
        \\[0.8pt] \noalign{\vskip 1pt}
        % 
        \multirow{1}{*}{{$^*$}DNS-SLAM~\cite{kunyi2023dns}}                    
        & 0 & 1 & 2 & 3 & 4                       
        \\[0.8pt] \noalign{\vskip 1pt}
        % 
        \multirow{1}{*}{{$^*$}SNI-SLAM~\cite{zhu2024sni}}   
        & 0.62 & 0.77 & 29.43 & 0.935 & 0.235 
        \\[0.8pt] \noalign{\vskip 1pt}
        %
        \multirow{1}{*}{Point-SLAM~\cite{sandstrom2023point}} 
        & 0.53 & 0.44 & 35.17 & \fs 0.975 & 0.124  
        \\[0.8pt] \noalign{\vskip 1pt}
    
        \hdashline \noalign{\vskip 1pt}
        \multicolumn{6}{l}{\cellcolor[HTML]{EEEEEE}{\textit{3D Gaussian Splatting}}} \\ 
        % 
        \multirow{1}{*}{SplaTAM~\cite{keetha2024splatam}} 
        & 0.41 & 0.67 & 33.55 & 0.971 & 0.090     
        \\[0.8pt] \noalign{\vskip 1pt}
        % 
        \multirow{1}{*}{Gaussian SLAM~\cite{yugay2023gaussian}}
        &  0 & 1 & 2 & 3 & 4                        
        \\[0.8pt] \noalign{\vskip 1pt}
        % 
        \multirow{1}{*}{MonoGS~\cite{matsuki2024gaussian}}
        & 0 & 1 & 2 & 3 & 4                         
        \\[0.8pt] \noalign{\vskip 1pt}
        
        \multirow{1}{*}{Ours} 
        & \fs 0.35 & \fs 0.39 & \fs 37.18 & 0.966 & \fs 0.046  \\
        
        \bottomrule
    \end{tabular}
    }
    \caption{Quantitative comparison on the Replica dataset.}
    \label{tab:replica_slam}
\end{table}

==> tab/replica_dataset.tex <==
\begin{table}[t]
    \centering
    % \setlength{\tabcolsep}{2pt}
    \renewcommand{\arraystretch}{1.05}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lccccccccc}
    \toprule
    \textbf{Method} & \textbf{O0} & \textbf{O1} & \textbf{O2} & \textbf{O3} & \textbf{O4} & \textbf{R0} & \textbf{R1} & \textbf{R2} & \textbf{Avg.}\\
    \midrule
    \multicolumn{10}{l}{\cellcolor[HTML]{EEEEEE}{\textit{Neural Implicit Fields}}} \\ 
    \multirow{1}{*}{NICE-SLAM~}     &    1.82   &    0.72   &    1.50   &    2.79   &    3.34   &    1.72   &    3.32   &    2.07   &    2.16    \\[0.8pt]  \noalign{\vskip 1pt}
    \multirow{1}{*}{Vox-Fusion~}    &    8.48   &    2.04   &    2.58   &    1.11   &    2.94   &    1.37   &    4.70   &    1.47   &    3.09    \\[0.8pt]  \noalign{\vskip 1pt}
    \multirow{1}{*}{SNI-SLAM~}      &    0.55   &    0.52   &    0.67   &    0.99   &    0.73   &    0.55   &    0.53   &    0.49   &    0.63    \\[0.8pt]  \noalign{\vskip 1pt}
    \multirow{1}{*}{DNS-SLAM~}      &           &    0.84   &    0.69   &           &           &    0.72   &    1.08   &    0.76   &            \\[0.8pt]  \noalign{\vskip 1pt}
    \multirow{1}{*}{Point-SLAM~}    &    0.38   &    0.48   &    0.54   &    0.69   &    0.72   &    0.61   &    0.41   &    0.37   &    0.53    \\[0.8pt]  \noalign{\vskip 1pt}
    
    \multirow{1}{*}{GO-SLAM~} 
     &  0.34  &  0.29 &   0.29   & \rd  0.32  &  0.30  &  \rd 0.39 & 0.39 & \rd 0.46& 0.35 \\
    [0.8pt]  \noalign{\vskip 1pt}
    %
    \multirow{1}{*}{Loopy-SLAM~} 
     &\fs 0.24  & \rd 0.24  & \rd 0.28 & \nd 0.26  &  0.40  &  \nd 0.29 & \rd 0.22  & \nd 0.35  & \nd 0.29  \\
    %
    [0.8pt]
    
    \hdashline \noalign{\vskip 1pt}
    \multicolumn{10}{l}{\cellcolor[HTML]{EEEEEE}{\textit{3D Gaussian Splatting}}} \\ 
    \multirow{1}{*}{SplaTAM~ 
    } 
     &  0.31  &  0.40   &  0.29   &  0.47   &  0.27   &  \nd 0.29  & 0.32  &  0.72 &  0.38  \\
    [0.8pt]  \noalign{\vskip 1pt}
    %
    \multirow{1}{*}{MonoGS~ 
    } 
     & 0.33  &  \fs 0.22  & 0.29    & 0.36    &  \nd 0.19  & \fs 0.25  & \fs 0.12 & 0.81  & 0.32  \\
    [0.8pt]  \noalign{\vskip 1pt}
    %
    \multirow{1}{*}{Gaussian-SLAM~ 
    } 
     & \rd 0.29  &  0.29  & \nd 0.22    & 0.37    &  \rd 0.23  &  0.41  &  0.30 & \nd 0.35  &\rd  0.31  \\
    [0.8pt]  \noalign{\vskip 1pt}
    %
    \multirow{1}{*}{{$^*$}Photo-SLAM~ 
    } 
    &  0.54  &  0.39   &  0.31   &  0.52   &  0.44   &   1.28  & 0.78  &  0.58 &  0.60  \\
    [0.8pt]  \noalign{\vskip 1pt}
    %
    \multirow{1}{*}{\textbf{\ours (Ours)}} 
     &\nd 0.28  & \fs 0.22  & \fs 0.17 & \fs 0.22  & \fs 0.16  &   0.49 & \nd 0.20  & \fs 0.30  & \fs 0.26  \\
    
    
    \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Tracking Performance on Replica~} (ATE RMSE $\downarrow$ [cm]). LC indicates loop closure. The best results are highlighted as \colorbox{tabfirst}{first}, \colorbox{tabsecond}{second}, and \colorbox{tabthird}{third}. \ours performs the best. $^*$Photo-SLAM~ is a \textit{decoupled} method using ORB-SLAM3~ for tracking and loop closure.}
    \label{tab:replica_tracking}
\end{table}
    

==> tab/replica_render.tex <==
\begin{table}[t]
    \centering
    % \setlength{\tabcolsep}{2pt}
    \renewcommand{\arraystretch}{1.05}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lccccccccc}
    \toprule
    \textbf{Method}                         &\textbf{O0}&\textbf{O1}&\textbf{O2}&\textbf{O3}&\textbf{O4}&\textbf{R0}&\textbf{R1}&\textbf{R2}&\textbf{Avg.}\\
    \midrule
    \multicolumn{10}{l}{\cellcolor[HTML]{EEEEEE}{\textit{Neural Implicit Fields}}} \\ 
    \multirow{2}{*}{NICE-SLAM~\cite{zhu2022nice}}         &      1.82 &      0.72 &      1.50 &      2.79 &      3.34 &      1.72 &      3.32 &      2.07 &      2.16  \\[0.8pt]  \noalign{\vskip 1pt}
    \multirow{1}{*}{Vox-Fusion~\cite{yang2022vox}}        &      8.48 &      2.04 &      2.58 &      1.11 &      2.94 &      1.37 &      4.70 &      1.47 &      3.09  \\[0.8pt]  \noalign{\vskip 1pt}
    \multirow{1}{*}{SNI-SLAM~\cite{zhu2024sni}}           &      0.55 &      0.52 &      0.67 &      0.99 &  \rd 0.73 &      0.55 &      0.53 &      0.49 &      0.63  \\[0.8pt]  \noalign{\vskip 1pt}
    \multirow{1}{*}{DNS-SLAM~\cite{li2024dns}}            &           &      0.84 &      0.69 &           &           &      0.72 &      1.08 &      0.76 &            \\[0.8pt]  \noalign{\vskip 1pt}
    \multirow{1}{*}{Point-SLAM~\cite{sandstrom2023point}} &  \fs 0.38 &      0.48 &      0.54 &      0.69 &  \nd 0.72 &      0.61 &  \rd 0.41 &      0.37 &  \rd 0.53  \\[0.8pt]  \noalign{\vskip 1pt}
    \hdashline \noalign{\vskip 1pt}
    \multicolumn{10}{l}{\cellcolor[HTML]{EEEEEE}{\textit{3D Gaussian Splatting}}} \\ 
    \multirow{1}{*}{SplaTAM~\cite{keetha2024splatam}}     &      0.53 &  \fs 0.23 &  \rd 0.36 &  \rd 0.43 &  \fs 0.64 &  \nd 0.33 &      0.44 &  \rd 0.35 &  \nd 0.41  \\[0.8pt]  \noalign{\vskip 1pt}
    \multirow{1}{*}{MonoGS~\cite{matsuki2024gaussian}}    &  \nd 0.45 &  \nd 0.37 &  \fs 0.27 &  \nd 0.26 &      0.97 &  \rd 0.39 &  \nd 0.34 &  \nd 0.26 &  \nd 0.41  \\[0.8pt]  \noalign{\vskip 1pt}
    % \multirow{1}{*}{Gaussian-SLAM~}                     &      0.29 &      0.29 &      0.22 &      0.37 &      0.23 &      0.41 &      0.30 &      0.35 &      0.31  \\[0.8pt]  \noalign{\vskip 1pt}
    \multirow{1}{*}{\textbf{Ours}}                        &  \rd 0.49 &  \rd 0.40 &  \nd 0.32 &  \fs 0.23 &      0.81 &  \fs 0.31 &  \fs 0.33 &  \fs 0.23 &  \fs 0.39  \\[0.8pt]  \noalign{\vskip 1pt}
    \bottomrule
    \end{tabular}
    }
    \caption{Comparison of tracking performance on Replica dataset~\cite{straub2019replica}. We report \textit{RMSE(cm)} for Absolute Trajectory Error (ATE) for different sequences. The best results are highlighted as \colorbox{tabfirst}{\textbf{first}}, \colorbox{tabsecond}{second}, and \colorbox{tabthird}{third}.}
    \label{tab:replica_render}
\end{table}
    
